Taming Diffusion Probabilistic Models for Character Control

We present a novel character control framework that effectively utilizes motion diffusion probabilistic models to generate high-quality and diverse character animations, responding in real-time to a variety of dynamic user-supplied control signals. At the heart of our method lies a transformer-based Conditional Autoregressive Motion Diffusion Model (CAMDM), which takes as input the character's historical motion and can generate a range of diverse potential future motions conditioned on high-level, coarse user control. To meet the demands for diversity, controllability, and computational efficiency required by a real-time controller, we incorporate several key algorithmic designs. These include separate condition tokenization, classifier-free guidance on past motion, and heuristic future trajectory extension, all designed to address the challenges associated with taming motion diffusion probabilistic models for character control. As a result, our work represents the first model that enables real-time generation of high-quality, diverse character animations based on user interactive control, supporting animating the character in multiple styles with a single unified model. We evaluate our method on a diverse set of locomotion skills, demonstrating the merits of our method over existing character controllers. Project page and source codes: https://aiganimation.github.io/CAMDM/

==> submission/0-abs.tex <==
\begin{abstract}

We present \name, 
%a generative model that takes a single or few example sequences and synthesizes, within a fraction of a second, diverse and high-quality sequences that resemble the examples. 
a generative model that ``mines'' as many diverse motions as possible from a single or few example sequences.
%
In stark contrast to existing data-driven methods,
which typically require long offline training time, are prone to visual artifacts, and tend to fail on large and complex skeletons,
\name inherits the training-free nature and the superior quality of the well-known \emph{Motion Matching} method.
%
\name can synthesize a high-quality motion within a fraction of a second, 
even with highly complex and large skeletal structures.
%\name partitions the example sequences into ``chunks''  and ``mines'' as many diverse motion chunks as possible, then novel motion is synthesized via generative motion matching. Thus, \name  inherits the training-free nature and the superior quality of the well-known motion matching.
%, which is the de facto state-of-the-art technique for character animation in the industry.
%
At the heart of our generative framework lies the generative motion matching module,
which utilizes the bidirectional visual similarity as a generative cost function to motion matching,
and operates in a multi-stage framework to progressively refine a random guess using exemplar motion matches.
%
In addition to diverse motion generation,
we show the versatility of our generative framework by extending it to a number of scenarios that are not possible with motion matching alone,
including motion completion, key frame-guided generation, infinite looping,
and motion reassembly.



\if 0
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % : spare sentences
% %%: comments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% 
%% strengths of our proposed method
We introduce a patch-based generative framework to synthesize novel motions from a few input sequences. Our method is conceptually simple, requires \textit{no training}, 
and can generate diverse, highly detailed motions within a split second.
%
%% show differences in previous works (GAN-based, statistical model, etc.)
%% 1:   without training
%% 2:   not data-driven, can learn from a single sequence
%% 3:   do not need ad hoc designs
%% 3.1: robust to different rotation representation
%% 3.2: can handle complex skeletons (NN meet performance degradation issues when the skeleton are complex)
%% 3.3: previous works require desired and specific skeletal structure (not sure, mentioned in GANimator)
%% 4:   explicit control
Existing generative models for motion are typically data-driven, requiring a long training stage, 
and ad hoc designs, such as rotation representation and skeletal operators, need to be utilized, 
which largely constrains their practicality in real-world applications.
%
%% illustrate our main idea
In this work, we re-investigate the classical 2D patch-based texture synthesis methods.
Our core idea is to inject generative capabilities into the classical patch-based model
and generate diverse results both on the temporal and skeleton dimensions hierarchically.
%
%% details of our method
Specifically, we start with an initial coarse guess, 
then a novel motion that is reassembled by exemplar patches is obtained using the nearest neighbor search.
The process is performed in a coarse-to-fine manner to capture varying levels of detail.
% Without the need of training or specialized designs,
% the advocated non-parametric framework allows generating diverse motions, 
% while preserving all the details of the input exemplar.
%
%% evaluation
We extensively evaluate our framework, showing that it achieves superior results over other methods, both qualitative and quantitative.
%
%% application
Our explicit framework can be easily adapted to a wide range of applications, including key-frame editing, looping, motion completion and diverse in-betweening.

\xl{to be updated.}
\fi

\end{abstract}

==> submission/1-intro.tex <==
\section{Introduction}

%Human motion is highly varied and continuous:
%it quickly adapts to various purposes, 
%and is capable of transitioning from almost arbitrary poses.
%
The generation of natural, varied, and detailed motions is a core problem in computer animation.
%
%On the other hand,
Acquiring large volumes of motion data via a motion capture (mocap) system or manually authoring sophisticated animations is known to be costly and tedious.
%
As such, motion datasets are generally limited, especially in terms of the diversity of style, skeletal structures, or creature types, which hamper the effectiveness of existing data-driven motion synthesis methods.
%
Advancing generative abilities of
synthesizing diverse and extensive motions from limited example sequences
has therefore become an important research problem.
%\xl{Here we convey why exemplar-based setting matters.}


% neural synthesis
In recent years,
deep learning 
%(a deep framework, PFNN, MANN, moglow, etc)
has taken the field of computer animation by storm.
Deep learning methods have demonstrated the ability to synthesize diverse and natural motions when 
training on large and comprehensive datasets~\cite{holden2016deep, pfnn, moglow, motionclip,raab2022modi, tseng2022edge}.
%
More encouragingly, the success was recently reproduced in an extremely reduced setting~\cite{ganimator},
where only one sequence is provided for training, yet, the neural network learns the sample's internal distribution,
and demonstrates the ability to synthesize diverse variants of the input example sequence.
%
%
Nevertheless,
neural motion synthesis methods carry several drawbacks that limit their applicability in practice:
(i) they require long training time;
(ii) they are prone to visual artifacts such as jittering or over-smoothing;
(iii) they do not scale well to large and complex skeleton structures.


%
%So,
% Still,
% it might be seemly that one shall foresee a storm in academia, 
% where deep learning would evolve and prevail as per usual.
%on exemplar-based motion synthesis,
%
%The deep learning area on exemplar-based motion synthesis is seemly upon us.
%
%\xl{Here for how existing work, mainly neural-based ones, solve the problem.}
%yet
%In this paper, we act in a diametrically opposite way.
In this paper, we explore an alternative approach to the problem.
We revisit the classical idea in computer animation \--- \emph{motion nearest neighbors}~\cite{motionfield},
which dates back long before the deep learning era and 
on which the state-of-the-art industrial solution for character animation \--- \emph{motion matching} \--- was founded~\cite{motionmatching}, delivering exceptionally high-quality motion synthesis.
%
%We are particularly attracted by the quality of motion this method produces.
%
Motion matching produces character animations that appear natural and respond 
to varying local contexts.
%Motion matching produces character animations that appear natural and respond 
%%to arbitrary control signals presented to them.
%to the exponentially growing number of different situations presented to them.
%,
%and is known for the quality of motion it produce.
%
%As human motion is highly varied and continuous,
%
Using a large mocap database as a local approximate of the entire natural motion space,
motion matching simply searches for a motion patch that best fits a given local context. 
%
%however,
%the original algorithm was simply to search in the database for a motion patch best fits the given local context.
%,
%and plays back the animation data stored in the database \emph{as-is}.
%
%This is, obviously, at variance with a generative model,
%which has a particular emphasis on capturing the data distribution across the whole database for drawing in-distribution samples afterwards.
%
The dependence on a large dataset is, however, at odds with our goal: we are after a generative model that ``mines'' as many \emph{diverse} motions as possible from a \emph{single} or \emph{few} examples.
%such as implicit distribution learned in~\cite{ganimator}
%\xl{to add: mm = big data approximates large continuous motion space, different goal -  so as to respond correctly to any control signal.
%while our goal is a generative model that fully tap the potential diversity in the data.}

%
Inspired by the work of \citet{dropthegan} in image synthesis,
we take the following insights for casting motion matching into our generative model and yield \emph{generative motion matching} (\name, pronounced "gem").
%
First,
to retain the motion quality of motion matching and inject generative capabilities,
we exploit bidirectional similarity introduced in~\cite{simakov2008summarizing}
%which serves the purpose of comparing the patch distribution between the exemplar and the synthesized motion,
as a new generative cost function for motion matching.
%we replace the cost function of motion matching
%with the bidirectional similarity introduced in~\cite{simakov2008summarizing},
%which serves the purpose of comparing the patch distribution between the exemplar and the synthesized motion.
%for comparing the patch distribution between the exemplar and the output,
%as a catalyst for casting the motion matching into a generative model.
%
The bidirectional similarity serves the purpose of comparing the patch distribution between the example and the synthesized sequence.
%
Specifically,
it encourages the synthesized sequence to contain only motion patches from
the example sequences, 
and vice versa,
the examples should only contain motion patches from the synthesis.
%
Consequently, no artifacts are introduced in the synthesis, 
and importantly, 
no critical motion patches are lost either.
%encourages the synthesized motion to contain only motion patches from
%the exemplar motions (“Visual Coherence”), and vice versa
%, the exemplar motions should contain only patches from the output 
%(“Visual Completeness”). 
%
Second,
we use a multi-stage framework to progressively synthesize a motion sequence that has minimal patch distribution discrepancy with the example,
capturing patch distributions from varying temporal resolutions.
%
%By minimizing the patch distribution discrepancy between the exemplar and the synthesized motion at multiple temporal resolutions in a coarse-to-fine generation,
%a motion that resembles the exemplar motions can be synthesized.
%
%The bidirectional similarity compares the patch distribution between the exemplar motions and the output during motion synthesis,
%playing as a catalyst that casts the motion matching into a generative model.
Lastly,
we utilize the observation that the generative diversity of GAN-based methods stems primarily from the unconditional noise input~\cite{dropthegan}:
we input noise to the coarsest synthesis stage, and achieve highly diverse synthesis results.
%\xl{How we are going to solve it, the conceptual difference. %we cast mm into a generative model: bidirectional similarity that compares distributions at multiple stages + noise adding randomness for diversity.}



%we argue that patch is better than neural-based in motion synthesis.
%On the primary generative task, i.e., diverse motion synthesis from examples,
We demonstrate that \name is more than competent in producing diverse motions from only a small set of input examples.
%
Notably, 
compared to existing works,
\name offers several advantages:
\begin{itemize}
\item 
\name runs very fast, without any pre-training.
A motion sequence can be synthesized within a fraction of a second.

\item 
\name inherits the appealing nature of motion matching, producing motions of high quality and fidelity.
%(evidenced by sharp movements in popping dance results).

\item
%Operating at the patch level,
\name scales smoothly to highly complex skeletons (see the character with 433 joints in Figure~\ref{fig:teaser}), where neural networks struggle~\cite{ganimator}.

\item
It is easy to extend \name to inputs with multiple sequences and encourage the synthesis to cover all examples, which is non-trivial for GAN-based methods~\cite{ganimator}.

\end{itemize}

%These are verified by extensive evaluations.
%
%Last,
In addition to diverse motion generation,
we also demonstrate the versatility of our generative framework by extending to an array of scenarios that are unachievable with motion matching alone, such as  
motion completion, key frame-guided generation, infinite looping, and motion reassembly, 
all enabled by the shared foundation of generative motion matching.
















\if 0

\todo{
may be a key point: argument for patch is better in motion generative model
}

%
%% =========================================================================
%% 1. Compared to patch-based image synthesis, patch-based methods are more suitable for motion synthesis. 
%%    As we actually do not concentrate on the diversity of the synthesized motions, but on the quality of the motion.
%%
%%
%%
%% =========================================================================

%% motivation
Our goal is to inject new vitality of diverse generation into the classical patch-based motion synthesis framework.
%% strengths comparing with NN-based methods
Different from generative neural networks, our non-parametric approach is simple yet effective, which can synthesize diverse novel motions from multiple exemplars within a second without training and ad hoc designs.
%% skeleton-aware components
Moreover, to fully facilitate the potential of exemplars, a novel skeleton-aware mechanism is introduced to 
% \plc{Agree that this is more like the intro part. But remember to add the applications enabled by skeleton-aware components when move to intro.}

\xl{below are some remarks.}

Motion synthesis is the holy grail in computer animation.
Because it is hard to have large scale mocap data, a promising direction is to synthesize from a few exemplar clips.

recent single-clip gan training, ganimator resorts to learn the internal distribution of a clip.
while success in demo more diversity emerged in the learning, they have some shortcomings: 1. long training time, 2. artifacts in motion deviate from the input, 3. hard to extend to more complex skeletons, 4.

We revive classical patch-based method, motion matching is a representative, that has been the de facto sota in locomotion synthesis. it is super fast, high-quality as the original motion patches are being simply reply to restore the data.
Inspire us to add add generative capability to mm, so generative motion matching.

our work, tech details.
skeleton-aware motion patches.
various setting.

the advantages of our method with generative motion matching: 1. super fast, 2. high quality motion (high frequency details also preserved), 3. work with highly complex skeletons, 4. work with multiple clips.
Easy to extend to more settings more applications.

we show our method produce sota results. visually super sharp!

\xl{more detailed version}
\fi

==> submission/2-related.tex <==
\section{Related work}
%
%% =========================================================================
%% 1. Motion
%%  1.1) traditional patch-based motion synthesis
%%  1.1) Motion texton
%%  1.2) Motion graph
%%  1.3) Motion field
%%  1.3) Motion matching
%%
%%
%%
%% 2. Image
%%  2.1) Texture synthesis
%%  2.2) Introduce 'Pyramid' to texture synthesis
%%  2.3) Nature image synthesis
%%      2.3.1) GAN-based methods
%%      2.3.2) Patch-based methods: (GPNN) Drop the GAN, (GPDM) patch distribution
%%
%%
%%
%% =========================================================================

\input{image/multi_stage_generation.tex}

We review the most related work on kinematics-based motion synthesis.
%
We also briefly cover recent advancements in image synthesis, particularly patch-based ones, from which we take inspiration.

%We review various relevant works on motion generation focusing on kinematics-based methods. We also briefly introduce the related works on texture synthesis, which is a very similar task to motion generation.

\paragraph{Motion Synthesis}
%Endowing diversity to existing motion data can date back to the work of \citet{perlin1996improv}, where the Perlin noise~\cite{perlin1985image} is added to the motion data for creating local diversity. 
Generating novel motions via diversifying existing ones can date back to the work of ~\citet{perlin1996improv}, where the Perlin noise~\cite{perlin1985image} is added to motion clips for obtaining variants with local diversity. 
%
\citet{pullen2002motion} show that mocap data can be used to enhance a coarse key-framed motion, by matching low-frequency patches and blending high-frequency details. 
%
\citet{motiontexture} 
construct a graph model by matching similar patches in the dataset,
%take another step with constructing a graph-like model by matching similar patches and organizing them within a large dataset, 
and create a stochastic model for generating random samples with local and structural variations.
Due to the use of a linear dynamics model, the model requires a large training dataset to achieve satisfactory results and faces a dilemma of quality and diversity.
%
Contemporarily, motion graphs~\cite{kovar2002motion, lee2002interactive, arikan2002interactive} use a similar discrete graph model while keeping it deterministic, namely a state machine, and demonstrate characters that respond interactively to the user input.
%the ability to generate motion that interactively responds to user input.
%
However, the discrete space inherently limits their agility and responsiveness. 
Hence, efforts on summarizing large datasets into statistical models have also been made since then ~\cite{pullen2000animating, brand2000style, bowden2000learning, grochow2004style, chai2007constraint, wang2007gaussian}. 
Instead of sorting the dataset into an organized but discrete structure or a statistical model, 
motion nearest neighbors~\cite{motionfield, levine2012continuous} operate directly on contiguous \emph{motion fields} to learn a control policy that interpolates the nearest neighbors of the current pose.
%
Following that,
~\cite{motionmatching} introduce Motion Matching, which is a method searching a large database of animations for the animation which best fits the given context. 
%
This method has quickly been
adopted by many studios due to its simplicity, flexibility, controllability, and the quality of the motion it produces~\cite{harrower2018real, buttner2019machine}.
%
%Surprisingly, without the need for learning controllers, motion matching~\cite{motionmatching} is able to generate high-quality motions with a rather simple patch matching and blending process, given the carefully crafted matching features and the user-specified control features. 
%
%Because of its simplicity and effectiveness, it stands for the most cutting-edge technology for interactive motion generation, and is keeping evolving with the effort from industry~\cite{harrower2018real, buttner2019machine}. 
%Since it directly matches and replays the motion from the mocap dataset, the generated result is extremely high-quality. 
Motion matching plays back the animation data
stored in the database as-is,
rendering it the de facto state-of-the-art in the industry.
% \plc{Also, refine the industrial standard. To add comments for motion matching - no training, high quality, but only for controlled generation and requires carefully crafted features.}
%
%
%%
%\wy{We may need to cite ~\cite{gesturematching22} here}
Nevertheless, its goal differs significantly from ours, as we target a generative model that synthesizes diverse motions from examples.

Recent advancements in deep learning also greatly impact the motion synthesis field. 
Early attempts
\cite{holden2015learning,holden2016deep} use deep neural networks to learn from animation data. 
Deep neural networks can learn a strong prior from a large dataset, solving many ill-posed generative tasks including motion prediction~\cite{fragkiadaki2015recurrent, pavllo2018quaternet}, motion in-betweening~\cite{harvey2020robust, duan2022unified, qin2022motion}, motion reassembling~\cite{motionpuzzle, Chimera}, text-guided motion synthesis~\cite{motionclip, mdm, zhao2023modiff}, etc. 
\citet{holden2015learning,holden2016deep} apply modern deep learning techniques for learning from animation data. 
%
Meanwhile, combining motion matching with deep learning has also resulted in variants that are computationally less expensive~\cite{holden2020learned} and more versatile~\cite{habibie2022motion}. 
%
Notably,
all these works require a large and comprehensive dataset for training.
%
More recently, \cite{ganimator}, the most related work to us, proposes to use a patch GAN-based~\cite{pix2pix2017, singan} approach to train a generative model with a single example. 
%It is particularly interesting for the community as the acquisition of mocap data is difficult. 
%Though the goal highly resembles ours, the long training time, 
%the lack of high-frequency results and being unable to deal with multiple training because of the not well-structure latent space limit its usage. 
Nonetheless,
this method struggles to produce results with sharp motions, and is not suitable for training with multiple examples due to the discontinuous underlining 
 latent space presented to it.
%
We show the superiority of our method over GANimator by an in-depth comparison in \Cref{sec:comparisons}.  
% \plc{Comments: training time, over-smoothed result, difficulty in handling multiple sequences.}
% \begin{itemize}
    % \item Perlin noise on animation~\cite{perlin1996improv}. 
    % \item Enhance key-framed animation with mocap data~\cite{pullen2002motion}.
    % \item Probalistic model with a large dataset: motion texton~\cite{motiontexture}
    % \item Motion graph~\cite{kovar2002motion, lee2002interactive, arikan2002interactive}
    % \item motion field~\cite{motionfield} sought to learn a control policy based on the linear combination space of nearest neighbors.
    % \item Contiguous character control with low-dimensional embedding~\cite{levine2012continuous}. \plc{We will ignore this one.}
    % \item Matching like crowd generation~\cite{lerner2007crowds}. \plc{This one is about trajectory generation, we will ignore this one.}
    % \item motion matching~\cite{motionmatching}, learned motion matching~\cite{holden2020learned}, motion matching for gesture synthesis~\cite{habibie2022motion}.
    % \item Deep learning: First work~\cite{holden2016deep}, ganimator~\cite{ganimator}
% \end{itemize}
% \paragraph{Motion Nearest Neighbors.}


\paragraph{Image Synthesis} 
Our work adopts several algorithmic designs from texture image synthesis, that shares a similar goal with motion synthesis. 
%We briefly review related methods in the image domain, particularly classical parametric free method. 
For an in-depth survey of this extensive body we refer readers to surveys \cite{wei2009state, barnes2017survey}.
%
%\citet{efros1999texture} propose a parametric free sampling solution for texture synthesis, by modeling it as Markov Random Field (MRF). Image quilting~\cite{efros2001image} achieves novel texture synthesis and texture transfer using the idea of matching and stitching. 
The image pyramid, also known as progressive generation~\cite{karras2018progressive} in deep learning, had been used in texture synthesis long ago. 
\citet{heeger1995pyramid, de1997multiresolution} use a Laplacian pyramid~\cite{burt1987laplacian} for texture synthesis, realizing progressive generation on the spatial frequency domain. \citet{wei2000fast} use a Gaussian pyramid for a similar purpose. \citet{multiscale} push the multi-scale generation to a new height,
where gigapixel-sized images with great details can be synthesized.
%spanning over multiple spatial scales. 
We also adopt the progressive synthesis, allowing our generative motion matching module to capture details of different levels. 
%Also influenced by the booming of deep neural networks, convolution neural networks~\cite{gatys2015texture} are used for texture synthesis. Another major milestone is marked by the proposal of generative adversarial networks (GANs)~\cite{goodfellow2014generative}, which is a very powerful tool for generating images with rich semantic information from a large dataset. \citet{bergmann2017learning} adapt the original GAN for texture synthesis using a tailored spatial GAN architecture. 
Progressive synthesis has also become popular in today's era of deep learning,
leading to impressive generative models that learn to progressively refine random noise into images resembling a single natural image. 
Specifically,
a series of GANs~\cite{goodfellow2014generative} are trained to capture the patch distribution of the example at varying scales.
%Although it is generally believed that GANs are data-hungry, 
%single example based GANs~\cite{shocher2019ingan, singan} proved that it is possible to learn from just a single example. Specifically, SinGAN~\cite{singan} exploits the rich information from the patches in the Gaussian pyramid. 
Following that, \citet{dropthegan} show that
bidirectional visual similarity~\cite{simakov2008summarizing} can serve the purpose of measuring the patch distribution discrepancy between the example and the synthesized image,
leading to diverse images of much higher quality and fast synthesis, compared to GAN-based methods.
%minimizing bidirectional similarity~\cite{simakov2008summarizing} with patched nearest neighbor is qualitatively on par with SinGAN~\cite{singan} and is much faster as it is training free. \citet{elnekave2022generating} achieve the same goal using optimization to minimize the sliced Wasserstein distance between the generated patches and the training patches.

% achives comparale performance with more delicated models~\cite{efros2001image,kwatra2003graphcut}.

% \begin{itemize}
    % \item parametric free sampling~\cite{efros1999texture}, Image quilting~\cite{efros2001image}
    % \item other approaches: Image Graphcut~\cite{kwatra2003graphcut}. \plc{We'll skip this one}%, CNN based~\cite{gatys2015texture}
    % \item Pyramid related: Laplacian pyramid (frequency domain)~\cite{heeger1995pyramid}, multi-scale~\cite{multiscale}
    % \item Modern patch based: GPNN (bidirectional similarity)~\cite{dropthegan}, sliced Wasserstein distance~\cite{elnekave2022generating}, SinGAN~\cite{singan}.
% \end{itemize}




% \paragraph{Visual summary.}
% we need the generative power of GPNN. Maybe just append to the end of MNN.

==> submission/3-method.tex <==

\section{Method}


\if0

Our patch-based method:
1. super computationally efficient
2. applicable to various skeletons, even super complex ones.
3. sota performance

%
%% Weiyu: I would like to place our framework using multiple input exemplars rather than one.
%%        1) I want to address that we have an explicit knob (alpha) for completeness trade-off, while GAN-like
%%           methods have no mechanism to enforce Completeness. So if we have multiple sequences (more than 5 or 10), 
%%           GANimator can not get high coverage score. (I will try to set an experiment to show this)
%%        2) Moreover, our framework is efficient enough to handle multiple sequences (10 clips in a total of 5000 frames).
%%           GAN-based methods have a linear training time increase. So we can claim the efficiency of our framework.
%%
%%
%
%% 
%% Compare to GANimator and other motion synthesis methods
%% 1:   very fast, and do not need training
%% 2:   not data-driven, can learn from a single sequence
%% 3:   do not need ad hoc designs
%% 3.1: robust to different rotation representation
%% 3.2: can handle complex skeletons (NN meet performance degradation issues when the skeleton are complex)
%% 3.3: previous works require desired and specific skeletal structure (not sure, mentioned in GANimator)
%% 4:   explicit control
We propose a general patch-based motion synthesis framework
that can synthesize novel motions with an extremely intricate skeleton 
from multiple exemplars within a second, \emph{without training and other ad hoc designs}.
% The whole framework is in a hierarchical structure and efficient, effective, and explicit to 
Our work is inspired by works in image generation~\cite{dropthegan, singan} and motion generation~\cite{ganimator} from a single exemplar.
In the following, we describe the motion representation and the main components of our skeleton-aware patch-based synthesis framework. 

Although our approach can take as input multiple motion sequences,
which not necessarily share a common skeleton,
in our coverage, to ease understanding of the algorithm, 
we mainly describe in single motion setting.

input T frames, output F frames. not necessarily the same. 
\fi


We elaborate details of our generative framework,
that can synthesize high-quality motions resembling given examples, in large quantities and varieties.
%
%Our method is highly computationally efficient, 
%does not require long-time offline training,
%and can generate a sample in a fraction of a second.
%
Although our method can take as input \emph{multiple} exemplar motions,
in our coverage,
to ease the understanding of the algorithm,
we mainly describe in the \emph{single} input setting.
%
Moreover, the synthesized motion does not need to match exactly the length of the example and can be of arbitrary length.
%
%
%More details of adapting our method to various settings are also presented at the end.

%%%%%%%%%%%%%%%% Motion Representation %%%%%%%%%%%%%%%%
\subsection{Motion Representation}
%
A motion sequence is defined by a temporal set of $\nbframein$ poses
that each consists of root joint displacements $\rootpos \in \realnum^{\nbframein \times 3}$ and joint rotations $\jointrot \in \realnum^{\nbframein \times \nbjoint \rotdim}$,
where $\nbjoint$ is the number of joints and $\rotdim$ is the number of rotation features.
%
Instead of directly using the global root displacements $\rootpos$, 
we convert $\rootpos$ to local root displacements $\rootdelta$,
that are temporal-invariant and calculated as the difference between every two consecutive poses.
%
The joint rotations are defined in the coordinate frame of their parent in the kinematic chain,
and we use the 6D rotation representation (i.e., $\rotdim = 6$) proposed by \citet{zhou6d}.
%as in~\cite{ganimator}.
%
%Empirically,
%our approach works considerably well with both the quaternion and 6D  rotation representation,
%and by default uses the former (i.e., $\rotdim = 4$) for simplicity and efficiency.
%
%This is apparently at variance with the findings in previous neural-based works that advise the 6D rotation representation~\cite{ganimator, zhou6d},
%and we shall demonstrate the robustness of our approach to both alternatives.


%
As human eyes are rather sensitive to implausible interactions between the end-effector and the ground,
existing neural-based methods usually establish geometric losses on the locations and velocities of the end-effectors, i.e., the foot contact loss~\cite{shi2020motionet, ganimator, mdm},
%
whereas 
our method does not demand such a design
as the internal structure of exemplar motion patches,
such as the high correlation between the end-effectors and the root motion,
are inherently preserved in the synthesis.
%
That said,
it is also trivial to incorporate foot contact labels as in~\cite{ganimator} into our representation for improvements in \emph{rare} cases,
where sliding feet could occur in the synthesis with large root-motion examples.
%
%To further mitigate rare foot sliding artifacts, particularly in the synthesis with large root-motion inputs, 
%we follow~\cite{ganimator} and incorporate binary contact labels of specific foot joints in our motion representation.
%
The contact label enables the IK post-process to avoid floating feet.
%
Specifically,
the contact labels $\contactlabel$ can be easily retrieved from the input motion by setting a threshold of the magnitude of the velocity. 
Assume the number of foot joints is $\ncontact$, for each foot joint at a timestamp, we calculate a binary vector and append it to the per-frame feature (See Figure~\ref{fig:patch_extraction} and~\ref{fig:match_and_blend}).
%forming a new metric space 
%$\motionmetric_{\nbframe} \equiv \realnum^{\nbframe \times \left( \nbjoint \rotdim + 3 + \ncontact \right)}$.
%Figure~\ref{fig:patch_extraction} and Figure~\ref{fig:match_and_blend} present details of using contact labels.

%
For convenience,
we let
$\motionmetric_{\nbframe} \equiv \realnum^{\nbframe \times \left( \nbjoint \rotdim + 3 + \ncontact \right)}$ 
denote the metric space of concatenated motion features of $H$ frames, 
$\motionfeatin \equiv \left[ \jointrot, \rootdelta \right] \in \motionmetric_{\nbframein}$ the original input motion features,
$\motionfeatin_i \in \motionmetric_{\nbframein_i}$ a corresponding downsampled version of the input,
$\motionfeatout \in \motionmetric_{\nbframeout}$ the synthesized motion features of $\nbframeout$ frames,
and 
$\motionfeatout_\idstage$ a corresponding downsampled version of $\motionfeatout$.

\if 0
%
%% character animation representation. As we use skeleton patches, so we should define the skeleton first.
A segment animation of an articulated character can be represented by a tuple 
$\animatoin = \left\{ \bone, \motion \right\}$,
where $\bone$ describes the static part, i.e., the rest pose of the skeleton,  with the parent-child offsets and 
$\motion$ represents the dynamic component that specifies the movement of each joint.
%h
%% motion representation
More specifically, a motion $\motion$ can be represented as a sequence of temporally coherent poses of length $\nframe$, using root joint translation
$\translation \in \mathbb{R}^{\nframe \times 3}$
and joint rotations 
$\rotation \in \mathbb{R}^{\nframe \times \njoint \times \nrotfeat}$, 
where $\njoint$ and $\nrotfeat$ are the numbers of joints and rotation features of the current character, respectively.

%
%% details of the motion representation
%% translation is defined in the world space, and then convert to velocity
The translation of the root joint is specified in the world coordinate and describes the global location of the character. 
To make the representation agnostic to the starting position, we use the initial global displacement $\translation_0$ and temporal local velocities $\velocity_i := \translation_i - \translation_{i-1}$, which is retrieved by the difference between two adjacent timesteps.

%$\translation = \left\{ \translation_0, \velocity\right\}$, where velocity $\velocity_i = \translation_i - \translation_{i-1}$ and $\velocity_0 = \velocity_1$ indicates the global translation difference between two adjacent timesteps. 

%\plc{Breifly motivate why velocity: translation invariant.} \wy{Done. I'm not sure how to illustrate \emph{translation invariant} properly. This sentence may need modification.}

% 
%% rotation representation, we do not have to use 6D rotation representation
The rotation of each joint is relative to its parent's coordinate according to the kinematic chain, specifically, the rotation of the root joint describes the global orientation. 
Representation of rotation plays an important role in motion synthesis, especially in neural-based methods~\cite{continuity}, which usually utilize 6D representation to prevent performance degradation caused by different rotation features.
On the contrary, our patch-based framework is robust to different rotation representations (see ablation study in Section~\ref{ablation}), so we choose unit quaternions by default ($\nrotfeat = 4$) for simplicity and efficiency.
\plc{How robust is our method? I'm a bit skeptical because the 6D representation can also benefit us since we are using average voting. }
\wy{I can not notice the visual difference between two rotation representations, I will try to validate it in experiments.}


%
%% We may not need foot contact labels, BUT we can post-process the synthesized motion using IK to get better performance.
Although our framework can produce convincing results even without post-processing of foot contact in most cases as evidenced in Section~\ref{postprocessing}, to further refrain from foot sliding artifacts, we introduce binary contact labels to the foot joints of each specific character. 
% To further refrain from foot sliding artifacts, we introduce binary contact labels to the foot joints $\foot$ of each specific character. 
Following \citet{ganimator}, the contact labels can be easily retrieved from the input motion by setting a threshold of the magnitude of the velocity. 
Assuming the number of contact joints is $\ncontact$, for each foot joint at the timestamp, we calculate a binary vector, in the form of $\contactlabel \in \mathbb{R}^{\nframe \times \ncontact}$.
%% maybe do not mention it below, or move it to experiments?


%
%% definition of motion feature, downsampled motion, and skeleton part animation
Let 
$\motionfeat \equiv \mathbb{R}^{\nframe \times \left( \njoint \nrotfeat + \ncontact + 3 \right)}$ 
denote the concatenated feature of the motion $\motion$, 
which consists of joint rotations $\rotation$, local velocities $\velocity$ and contact labels $\contactlabel$.
A separate initial root position $\translation_0$ is saved to recover motions in world space.
% %
% %% this may move to 'Multi-scale Generation' section?
% A downsampled version of $\mootion$ is denoted by $\motion_{\nframe_{i}}$, 
% where $\nframe_{i} \subset \nframe$ is partial sequential samples of time.
% %
% %% this may move to 'Skeleton-aware Patches Extraction' section?
% In addition, we denote the part skeleton animation of a character to
% $\partanimatoin = \left\{ \partbone, \partmotion \right\}$,
% where $\partbone \subset \bone$ is the sub-tree of the character tree graph and $\partmotion \subset \motion$ is the corresponding motion.
\fi


%%%%%%%%%%%%%%%% Multi-scale Generation %%%%%%%%%%%%%%%%
\subsection{Multi-stage Motion Synthesis}
%
Figure~\ref{fig:overview} presents the overall pipeline of our approach,
which consists of $\nbstage$ stages to progressively synthesize a motion of $\nbframeout$ frames.
%
Specifically,
given an input motion,
we build an exemplar pyramid $\{ \motionfeatin_1, ...,  \motionfeatin_\nbstage \}$,
where $\motionfeatin_\nbstage = \motionfeatin$ is the original input sequence and $\motionfeatin_{\idstage} \in \motionmetric_{\nbframein_\idstage}$ is $\motionfeatin_{\idstage+1}$ downsampled by a factor $\downsamplef > 1$.
%
Then,
a synthesis pyramid $\{ \motionfeatout_1, ..., \motionfeatout_\nbstage \}$,
where $\motionfeatout_\nbstage \in \motionmetric_\nbframeout$ is the final synthesized sequence of $\nbframeout$ frames and $\motionfeatout_{\idstage} \in \motionmetric_{\nbframeout_\idstage}$ is an intermediate sequence of $\nbframeout \cdot \downsamplef^{\idstage - \nbstage}$ frames,
will be synthesized in a coarse-to-fine manner, starting from the coarsest stage and up to the finest.
%
At each stage $\idstage$,
the generative motion matching module (Section ~\ref{sec:patch_generation}) takes in an upsampled version of the output from the preceding stage as the initial guess, $\tilde{\motionfeatout}_{\idstage} = \motionfeatout_{\idstage-1} \upsample$,
refines it with exemplar motion patches in $\motionfeatin_\idstage$,
and outputs a finer motion sequence $\motionfeatout_\idstage$.
%
Note that
the synthesis
at the coarsest stage is purely generative,
as
the input is merely a noise drawn from a Gaussian distribution,
i.e.,
$\tilde{\motionfeatout}_1 \sim \mathcal{N}(\mu,\,\sigma^{2}) \in \motionmetric_{\nbframeout_1}$.


\if 0

%
%% overview
% \plc{This subsection needs a bit more work.}
\wy{It's indeed kind of a rush. I will refine it according to the comment.}
Figure~\ref{fig:overview} shows the overall architecture of our patch-based synthesis framework. 
As in previous works~\cite{multiscale, dropthegan, singan}, our framework employs a hierarchical process, 
in which the synthesized motion evolves from coarse to fine.
%
%% WHY we use multi-scale generation
In this pyramidal pipeline, 
we have the capability to capture and reproduce motions with different sizes of receptive fields varying over scales,
which allows us to access global diversity while maintaining local continuity.
\plc{We need to be more careful about the phrasing here. We can get back when we have a more polished intro.}

%  How the multi-scale generation is performed

%
%% build the pyramid for multi-scale generation
%% NOTE: GANimator set the number of the pyramid to 7. We do not constrain the number of the pyramid, so I do not mention the depth of the pyramid here. (will be mentioned in the patch extraction section to fit the patch size)
The input motions need to be organized in a hierarchical fashion for the purpose of multi-scale generation. 
Given $\nmotion$ examplar motions  $\left\{ \motion^i \right\}_{i = 1}^\nmotion$, 
we build a pyramid 
$\left( {{\motion^i}_{\nframe_1}}, {{\motion^i}_{\nframe_2}}, ...,{{\motion^i}_{\nframe_N}}, \right)$ 
% for each motion $\motion^i \in \left\{ \motion^i \right\}_{i = 1}^\nmotion$, 
for each motion $\motion^i$ in exemplars, 
where $\motion_{\nframe_{i}} = \downarrow^\upsampleratio\motion_{\nframe_N}$ 
is downscaled version of motion $\motion_{\nframe_N}$ with scaling $\upsampleratio$. 
% \plc{What is a partial sequential sample? It's not clear to me how are the $M^i_{T_i}$ constructed. By downsampling the examplar? The examplar is $M_{T_1}$ or $M_{T_N}$?}
\plc{The definition of $\{T_j\}$ is missing. I would suggest simply using $M_j$ to make it easier to read. Plus I think you'll need a set of $\{T_j\}$ for each $M^i$ (results something like $M^i_{T_j^i}$)}
% \wy{(Done) I fixed it. Actually, this section is kind of rough :(.}
%
%% use random noise as input
% Starting with an initial coarse guess $\synthesis_0$ produced by adding Gaussian noise
% $z_0 \sim \mathcal{N}(\mu,\,\sigma^{2})$
% to the concatenated input motions, 
Then, starting with an initial coarse guess $\synthesis_0 := M_0 + z_0$, 
where $z_0 \sim \mathcal{N}(\mu,\,\sigma^{2})$ is Gaussian noise.
\plc{$M_0$ not defined?}
% \plc{We should specify what is the ``concatenated input motions''. I think it's better to put this behind the motion pyramid and use notations to define $S_0$. E.g. $S_0 := M_0 + z_0$} \wy{I agree with it. Done.}
our framework updates and upsamples the motion to the finest resolution in a coarse-to-fine manner with $N$ stages.
In practice, 
we calculate $\nframe_{i} = {\uparrow^\upsampleratio}{\nframe_{i-1}}$, 
where $\uparrow^\upsampleratio$ is an upsampling linear interpolator with the same $\upsampleratio$.
% which is set to $4/3$ by default. \wy{Maybe $\upsampleratio = 4/3$ should move to pyramid construction or implementation details?}
%% TODO: I want to address that our method is robust to different hyperparameters, compared to the NN-based method.
% A downsampled version of $\mootion$ is denoted by $\motion_{\nframe_{i}}$, 

%
%% the input and the output at each stage
Except for the coarse stage,
each stage receives an initial guess $\widetilde{\synthesis}_n$ upsampled from the previous stage:
$\widetilde{\synthesis}_n = {\uparrow^\upsampleratio}{\synthesis_{n-1}}$ using the same upscale factor $\upsampleratio$
and then produces a refinement of the input motion using \textit{Patch Nearest Neighbor Field} module.

\fi

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{image/patch_extraction.pdf}
  \caption{
  Skeleton-aware motion patch extraction.
  %
  The skeleton is partitioned into several overlapping skeletal parts (two coloreds on the left),
  with which the full-body motion can be split into a set of partial-body motions accordingly.
  %
  Then motion patches (yellow boxes) with a temporal size of $\patchsize$ frames can be extracted from each partial-body motion.
  %Given a character, we divide the full-body motion into groups of partial skeletal motions. For each motion, we extract patches with size $\patchsize$ and stride $\stride$.
  }
  \label{fig:patch_extraction}
\end{figure}



%%%%%%%%%%%%%%%% Skeleton-aware  Patch Nearest Neighbor Field %%%%%%%%%%%%%%%%

\subsection{Generative Motion Matching}
\label{sec:patch_generation}
%
Typically,
patch-based image synthesis consists of three steps, namely the patch extraction, nearest neighbor matching, and blending,
that work in sequence to produce a converging result in multiple iterations.
%
% We take a similar practice that includes algorithmic designs specific to our task.
Our method follows a similar approach but with algorithmic designs specific to our task.
%
Specifically,
at each stage $\idstage$,
the following steps are invoked sequentially during $\nbiter$ iterations.




\paragraph{Skeleton-aware Motion Patch Extraction.}
%
A motion patch can be
defined trivially as a sub-sequence of $\patchsize$ consecutive frames in the example sequence,
which is a common practice in motion synthesis~\cite{ganimator, motionmatching}.
%
While our approach can simply work with this definition,
we further propose to extract skeleton-aware motion patches from the motion sequence,
which decomposes the skeleton into multiple sub-sets, 
i.e., skeletal parts,
instead of treating it as a whole,
and eventually leads to more \emph{diverse poses}.
%
Specifically,
let $\skeleton$ denote the skeletal tree used by the example full-body motion $\motionfeatin_\idstage$,
a set of skeletal parts 
$\{ \skeletalpart_1, ..., \skeletalpart_\nbpart \}$,
where $\skeletalpart_\idpart \subset \skeleton$ is a sub-tree of the whole skeleton and has $\nbjoint^{\idpart}$ joints,
can be defined to divide the full-body motion into a set of partial-body motions $\{ \partialmotion^1_\idstage, ..., \partialmotion^\nbpart_\idstage \}$,
from which we crop sub-sequences of $\patchsize$ frames with stride size $1$ as our motion patches (See Figure~\ref{fig:patch_extraction}).


\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{image/matching_and_blending.pdf}
  \caption{
  Generative matching and blending. 
  Each motion patch in the initial guess 
  finds the best-matched motion patch in the example motion,
  according to the normalized distance matrix.
  Then we blend the overlapping matched patches to form a novel partial motion. 
  Finally, we blend multiple resultant partial motions to get the final full-body motion (see right). 
  }
  \label{fig:match_and_blend}
\end{figure}

% how to get sub parts
Usually,
skeletons across different animations do not necessarily follow specific rules and can be of extremely high variability,
for example,
bipeds vs. hexapods, 
a pure biological skeleton vs. one with more artistic joints, etc.
Hence,
our approach allows the user to manually divide the whole skeletal structure into sub-parts with overlapping joints, similar as in~\cite{motionpuzzle, Chimera}.
% \wy{maybe 'Learning Virtual Chimeras by Dynamic Motion Reassembly' ?}
\if 0
%
On the other hand,
when the skeletal structure is relatively simple,
an automatic strategy can also be derived based on the skeleton-aware convolution operator introduced in~\cite{aberman2020skeleton} to split the skeleton into sub-parts,
for which we shall also showcase in the experiment section.
\fi






\paragraph{Generative  Matching.}
%
Let $\qset$ denote the set of motion patches extracted from $\tilde{\motionfeatout}_{\idstage}$,
$\kset$ the set of motion patches extracted from the example motion $\motionfeatin_{\idstage}$.
We calculate pairwise patch distance matrices using squared-$L2$ distance,
which provides the foundation for the measurement of the similarity between each exemplar motion patch and each synthesized motion patch.
%
Note that the patch distance matrix is calculated \emph{per} skeletal part:
\begin{equation}
\begin{gathered}
   \dist_{i,j}^{b} = \| \qset_{i}^{b} - \kset_{j}^{b} \|^2_2,
   % \dist_{i,j} = \frac{1}{\npart} \sum_{b=1}^{\npart}{|| \qset_{i}^{b} - \kset_{j}^{b} ||^2},
   \label{eq:patch_dist_matrix}
\end{gathered} 
\end{equation}
where $\qset^{\idpart}$ and $\kset^{\idpart}$ denote the set of motion patches extracted from corresponding partial-body motions.
%$\motionfeatout^\idpart_{\idstage}$ and $\partialmotion^\idpart_{\idstage}$.
%
Then, the bidirectional similarity as in \cite{simakov2008summarizing, dropthegan} is introduced to encourage
that all exemplar motion patches appear in the synthesis and all motion patches in the synthesis do not deviate from the example,
i.e., high completeness and coherence.
%This is particularly useful when the input has multiple motion clips,
This is achieved by normalizing the distance matrices using a per-key factor:
\begin{equation}
\begin{gathered}
   \simi_{i,j}^{b} =  \frac{\dist_{i,j}^{b}}{(\alpha + \min_{\ell}(\dist_{\ell,j}^{b}))} ,
\label{eq:distance_metric}
\end{gathered} 
\end{equation}
where $\alpha$ controls the degree of completeness,
and smaller $\alpha$ encourages completeness.




\paragraph{Blending.}
For each motion patch in $\qset^b$, we find its nearest (as defined by Equation~\ref{eq:distance_metric}) motion patch in $\kset^b$, 
and then blend the values of collected motion patches using average voting,
forming a synthesized partial-body motion $\bar{\motionfeatout}^b$.
%% blending on the skeletal dimension
Finally,
we average the values over overlapping joints between skeletal parts
to assemble all synthesized partial-body motions into the final result $\motionfeatout_\idstage$ (See Figure~\ref{fig:match_and_blend}).















\if 0

%
%% illustrate the main stages in patch-based synthesis
Typical patch-based image synthesis consists of three stages\plc{Here ``stage'' confuses the ``stages'' for the pyramid. It's better to use something else (maybe steps)}, 
namely the patch \emph{extraction}, \emph{matching}, and \emph{blending}.
\pl{We take a similar approach in our framework}. More specifically,
the \emph{extraction} divides the input query and exemplar into patches for further distance calculation and composition,
the matching finds the most suitable patch from the exemplar patches for each in the query,
and the latter blends the values of overlapped matched patches.
%% How to optimize. EM-like algorithm
The \emph{matching} and \emph{blending} stages are performed iteratively with $\nitr$ times,
to enforce the similarity between the internal statistics of the query and exemplar by an EM-like algorithm.
Specifically, details of each stage proceed as follows:





\paragraph{Skeleton-aware Patches Extraction.}
%
%% WHY we extract skeletal patches
To acquire diversity on both temporal and spatial dimensions,
we divide the skeleton into \emph{overlapping} patches and synthesize them individually,
significantly increases the range of synthesized motions.
More intriguing synthesized motions and applications can be found in ~\Cref{randomgeneration} and ~\Cref{reassembly} as evidence.
%% more details 
%
%% define the partial animation
Here, we denote a part skeleton animation of a character to
$\partanimatoin_i = \left\{ \partbone_i, \partmotion_i \right\}$,
where $\partbone_i \subset \bone$ is the sub-tree of the character tree graph and $\partmotion_i \subset \motion$ and is the corresponding motion.
As illustrated in Figure~\ref{fig:patch_extraction},
we divide the full-body motion $\motion$ into a set of partial motions
$\partmotion = \left(\partmotion_1, \partmotion_2, ...,\partmotion_{\npart} \right)$, 
where $\npart$ is the number of skeleton parts.
Then we concatenate the feature for each skeletal patch and denote it by $\partmotionfeat$.
Each motion feature in $\partmotionfeat$ has a subset of joint rotations and contact labels,
and the skeletal patch which contains a root joint inherits the local velocities of the full-body motion.

%
%% HOW to extract skeletal patches
%% 1, HOW to split the skeleton
%%  1) manually split
%%  2) for a simple and well-defined skeleton, we can automatically split it
%
%% manually split the skeleton
Many strategies can be utilized to extract skeletal patches, 
users can manually divide an intricate skeleton by preference
%
%% automatically split the skeleton 
%% weiyu: We may not mention the automatic splitting strategy as it is not trivial
and we also introduce an automatic splitting strategy for plain and well-defined skeletons.
Follow the work of \citet{aberman2020skeleton}, a skeleton structure can be treated as a tree-graph 
and the distance between two nodes can be calculated in the tree representation.
Starting from a leaf node, 
we collect joints whose distance is equal or less than the distance threshold $d$ to form a skeletal patch,
then we collect the next patch using a stride $s_{\text{skeleton}}$ until traversing the whole tree.
%% HOW to handle the contact joints
Specifically, the movements of contact joints need to be constrained to prevent foot sliding artifacts.
We calculate the minimum connected subgraph containing a set of all contact joints of the skeleton tree-graph
and treat all the joints in the subgraph as a whole group.

%
%% HOW to extract temporal patches
Thus, the input exemplar motions $\exemplar_n$ at stage $n$ can be represented as 
$\exemplar_n = \left( \partmotionfeat^1_{\nframe_n},  \partmotionfeat^2_{\nframe_n}, ..., \partmotionfeat^I_{\nframe_n} \right)$.
Patches with size $\patchsize$ in $\exemplar_n$ are extracted to form a query patch set $\qset$ using stride $\stride_{temporal}$ 
and ones with the same protocol in $\exemplar_n$ form a key set $\kset$.
%
%% weiyu: (Not sure) We may simply mention why do not use a skeleton pyramid here
% To keep the simplicity and versatility, we do not build a pyramid for the skeleton.







\paragraph{Match Patch Nearest Neighbors.}
%
%% first we calculate the distance between two sets using L2 distance
For each skeletal patch, 
we calculate the pairwise distance matrices using $L2$ distance individually,
which provides the foundation for the measurement of the similarity between query patch set $\qset$ and key patch set $\kset$.
\begin{equation}
\begin{gathered}
   \dist_{i,j}^{b} = \| \qset_{i}^{b} - \kset_{j}^{b} \|^2,
   % \dist_{i,j} = \frac{1}{\npart} \sum_{b=1}^{\npart}{|| \qset_{i}^{b} - \kset_{j}^{b} ||^2},
\end{gathered} 
\end{equation}
where $\qset^{b}$ and $\kset^{b}$ is the $b$-th skeletal patch.

%
%% completeness/diversity knob introduced by bidirectional similarity
Then, the bidirectional similarity proposed by \citet{simakov2008summarizing} and \citet{dropthegan} is introduced to control the degree of completeness in the synthesis,
which is achieved by normalizing the distance matrices $\dist$ using a per-key factor.
\begin{equation}
\begin{gathered}
   \simi_{i,j}^{b} =  \frac{\dist_{i,j}^{b}}{(\alpha + \min_{\ell}(\dist_{\ell,j}^{b}))} ,
\end{gathered} 
\end{equation}
where $\alpha$ provides an explicit knob for a trade-off between completeness and diversity
and smaller $\alpha$ encourages completeness.






\paragraph {Blend Matched Patches.} 
%
%% blending on the temporal dimension
For each query patch $\qset_i^b$ in the $b$th skeletal patch, we find its nearest patch in $\kset_l^b$, 
then blend the matched values of overlapping patches using average voting to form a synthesized partial motion $\synthesis_n^b$.
%% blending on the skeletal dimension
We eventually assemble all partial motions to get the final $\synthesis_n$, 
with the averaged values of overlapping joints.
\fi







\subsection{Extension to More Settings}
\label{sec:more_setting}
% TBA.
% multiple clips, with contact labels, and longer sequence

%
%While the description above has presented a simple yet effective method for diverse generation from a single sequence,
%
Our method can also be easily extended for various settings.
%, as demonstrated in the experiment section.



%%
\emph{Skeleton Partition for Motion Patches.}
In addition to the skeleton-aware motion patch defined above,
our method can also work with the traditional definition of a motion patch, i.e., treating the skeleton as a whole and then extracting $\patchsize$ consecutive poses.
%
\if 0
On the other hand,
when the skeletal structure is relatively simple,
an automatic strategy can also be derived based on the skeleton-aware convolution operator introduced in~\cite{aberman2020skeleton} to split the skeleton into sub-parts,
for which we shall also showcase in the experiment section.
\fi






\emph{Multiple Examples.}
As aforementioned,
our method can not only be applied to a single motion input but also works with multiple sequences of different numbers of frames.
%
This can be achieved by simply extracting motion patches from all input motions to form the set of exemplar patches used in Equation~\ref{eq:patch_dist_matrix}.
%
% Under this setting,
% the completeness control knob $\alpha$ is particularly important to encourage all motion patches across examples being used in the output.
In this setting, the completeness control knob $\alpha$ plays a crucial role in ensuring that all motion patches across examples are utilized in the output.





\emph{Heterogeneous Skeletons.}
Interestingly,
under the setting of multiple examples,
the skeletons across different motions do not necessarily share the same one.
%
For example, 
we can take motion clips of a monster and a zombie, 
and synthesizes a moving Frankenstein, 
via harmonizing different partial-body motions extracted from these two creatures.
\if 0
we can take motion clips of a human and a horse, 
and synthesizes an animation of a centaur, 
via harmonizing different partial-body motions extracted from these two creatures.
\fi
%To this end,
%we simply allow the user to split the skeleton of each input creature,
%manually specify the skeletal parts of interest to be used in the generative motion matching and blending.
%
%We then synthesize the novel motion for each skeletal part, 
%and finally, combine them to form the final motion of a new creature.
%
To achieve this, the user can split the skeleton of each input with overlap and manually specify the skeletal parts of interest to be used in the generative motion matching and blending. 
The overlapping region plays a crucial role in bridging different skeletal parts during the generation process. 
Then, our method can synthesize the novel motion for the new creature by combining the partial-body motions as discussed in Section~\ref{sec:patch_generation}.

\if 0

%%
\emph{Contact Labels.}
To further mitigate rare foot sliding artifacts, particularly in the synthesis with large root-motion inputs, 
we follow~\cite{ganimator}
and incorporate binary contact labels of specific foot joints in our motion representation.
%
The contact label enables the use of an IK post-process to avoid floating feet.
%
Specifically,
the contact labels $\contactlabel$ can be easily retrieved from the input motion by setting a threshold of the magnitude of the velocity. 
Assume the number of foot joints is $\ncontact$, for each foot joint at a timestamp, we calculate a binary vector and append it to the per-frame feature, 
forming a new metric space 
$\motionmetric_{\nbframe} \equiv \realnum^{\nbframe \times \left( \nbjoint \rotdim + 3 + \ncontact \right)}$.
Figure~\ref{fig:patch_extraction} and Figure~\ref{fig:match_and_blend} present details of using contact labels.
\fi

%More applications supported are shown in the experiment section.




\if 0
%% 
\paragraph{Multiple Clips}
As mentioned, our framework can be trivially extended to multiple inputs as shown in Figure~\ref{fig:overview},
enabling us to acquire more diversity in skeletal and temporal dimensions.
\wy{I want to address 1) different skeletons. 2) the explicit completeness knob here, which is different from the other methods.}
The skeletons of the input motions do not need to be exactly the same, we can combine different motions of different characters to obtain a \emph{frankenstein monster}, as shown in ~\ref{reassembly}.
%%
Moreover, different from the other methods, the completeness control knob provides an explicit way to evenly resemble all the exemplars.
%% details
Specifically,
given a set of exemplar motions 
$\left\{  \motionfeatin^1, \motionfeatin^2, .., \motionfeatin^I \right\}$,
we build a pyramid for each motion $\motionfeatin^i$ with the same factor $\downsamplef$.
The depth of all pyramids is shared with all motions, 
which is calculated by the minimal length of all motion sequences.
The length of the shorted exemplar motion at the coarsest stage
usually $2 \sim 3$ times of the patch size $\patchsize$.

\paragraph{Contact Labels}
%
%% 
To further refrain from \emph{rare} foot sliding artifacts, following \cite{ganimator},
we can naively incorporate the binary contact labels to the foot joints of each specific character for post-processing.
The contact labels can be easily retrieved from the input motion by setting a threshold of the magnitude of the velocity. 
Assume the number of contact joints is $\ncontact$, for each foot joint at the timestamp, we calculate a binary vector, in the form of a novel metric space 
$\motionmetric_{\nbframe} \equiv \realnum^{\nbframe \times \left( \nbjoint \rotdim + 3 + \ncontact \right)}$.
Figure~\ref{fig:patch_extraction} and Figure~\ref{fig:match_and_blend} present details of the use of contact labels.



\fi


==> submission/4-exp.tex <==


\begin{figure*}[th!]
  \centering
  \includegraphics[width=\linewidth]{image/random_generation_2.pdf}
  \caption{
  %
  From a single example,
  our framework generates, within a second, diverse motion sequences for even highly complex and large skeletons, including the animation of the clothes and the wings.
  %
  Please refer to the accompanying video for more animation results. 
  }
  \label{fig:randomgenetaion}
\end{figure*}


\section{Experiments}
\label{experiments}




%
%% =========================================================================
%% bullet points:
%%       1) effective
%%          1.1) w/o training 
%%          1.2) fast inference
%%       2) robust
%%          2.1) can handle complex skeletons
%%          2.2) robust to different rotation representations
%%          2.3) w/o post-processing
%%       3) preserve motion details, may need a velocity figure
%%       4) we have an explicit mechanism to ensure the completeness
%%       5) skeleton-aware component
%% =========================================================================
\if 0
%% Weiyu: I'm not sure how to evaluate the skeleton-aware component
%
We extensively evaluate our proposed framework using a rich variety of motions.
%
%% details about the chosen exemplars
Some are with extremely intricate skeletons (with more than 400 joints) are commonly used in real production
and others are rhythmic dance choreographies like hip-pop,
possessing varying degrees of complexity in terms of spatial and temporal.  % Weiyu: 'temporal' may not be very proper?
%% briefly introduce some subsections in experiments
In the following, we present the qualitative evaluation of our results,
showing the effectiveness and efficiency compared to other statistical or neural-based generation methods.
We then demonstrate the flexibility of our framework through a bunch of experiments with different settings.
More intriguing visual results can be found in our accompanying video.
\fi
We evaluate the effectiveness of our method on example-based motion synthesis, compare to other motion generation
techniques,
and demonstrate its versatility by applying it in various settings and applications. We highly recommend readers refer to the accompanying video for more qualitative evaluations.
%
\emph{Code and data will be released, upon paper publication, to ease the understanding of our implementation and facilitate future studies.}



%\xl{
%Random gen results (various skeletons) and comparison (fair comparison, all with 65 joints)
%1. in basic setting: no skeleton-aware + single clip 
%2. two figures: one for our gallery + one for comparison.
%}

\paragraph{Data.}
%
We collected a diverse set of example animations featuring varied motion styles and highly complex and large skeletal structures from Mixamo~\shortcite{mixamo} and Truebones~\shortcite{truebones}.
%
The motion styles we experimented
with include sharp motions of a popping dance, subtle motions of fanning wings, etc.
Some examples are authored with highly sophisticated skeletal structures, such as the 433-joint and 143-joint skeletons as visualized in Figure~\ref{fig:randomgenetaion}.
%
The number of frames ranges from 140 to 1000 frames at 30 fps.
 
%% data setting
%We collect a set of motion sequences mainly from Mixamo~\shortcite{mixamo} and Truebones~\shortcite{truebones}.
%
%The examples come with various skeletons of different complexity,
%and the number of frames ranges from 140 to 1500 frames (30 fps).
%
%% briefly introduce time consumption

\paragraph{Implementation Details.}
%
%% hardware setting
%
Our framework is lightweight and does not require any training.
Due to its simplicity and efficiency,
we simply implement our method with Python.
%
We also develop an add-on in the open source software Blender~\cite{blender}, which is ready to take animations from users and synthesizes diverse and high-quality variants.
%We implement our framework in PyTorch for parallel computation of the similarity matrices.
%Our method is lightweight, without heavy training.
In our implementation,
a motion sample with around 1000 frames can be generated in $\sim0.2$s with an Apple M1 CPU or $\sim0.05$s with a modern GPU (NVIDIA V100).
By default, we run experiments using an Apple M1 CPU,
except that the comparison experiments are conducted using an NVIDIA V100 GPU for fair comparisons with neural network-based methods. 
%
%% hyperparameters setting: pyramid depth, noise, patch size/stride, (how to split skeleton?), alpha, number of steps
% The pyramid depth $N$ is set according to the length 
% The pyramid depth $N$ is set according to the minimal frames of all exemplar motions.
% independent variables: the ratio of the patch size to the length of the minal frames (K)
% The patch size $\patchsize$ is set to cover $K=1/8\sim1/2$ of the synthesized motion $\tilde{\motionfeatout}_1$ at the coarsest stage,
% and then synthesized motion is gradually upsampled until it reaches the final length.
%Choosing the scale from which to start plays an important role in multi-scale architecture,
%and 
We set the length of $\motionfeatin_1$ at the coarsest stage to $K$ times the patch size $\patchsize$. 
Thus the receptive field (a similar concept as in the image) always occupies the same proportion of example motions with different lengths.
%
Then, $\motionfeatin_1$ is gradually upsampled using the factor $\downsamplef$
until it reaches the final length of $\motionfeatin_S$.
% We may do not mention the multiple examples?
% For multiple input examples, we choose the shortest example as
Unless otherwise specified,
we use a  patch size $\patchsize=11$, $K=4$, a completeness control knob $\alpha=0.01$ and a number of iterations $\nbiter = 5$. These are the empirically best hyper-parameters we have found. For more discussions on the hyper-parameters, please refer to the supplementary material.
%Please note that our method is robust to varying hyper-parameters to some extent, 
%more experiments can be found in Section ~\ref{hyperparameters}.




%%%%%%%%%%%%%%%% Random Generation %%%%%%%%%%%%%%%%
\subsection{Novel Motion Synthesis}
\label{randomsynthesis}


%
%\wy{I want to address the complexity of skeleton / skeleton-level diversity / synthesized details / explicit coverage in this section.}
We first evaluate the performance of our framework on novel motion synthesis,
and compare it to a classical statistical model and recent neural-based models, namely MotionTexture~\cite{motiontexture}, acRNN~\cite{acrnn} and GANimator~\cite{ganimator}.

\paragraph{Settings}
Although our method can use multiple inputs, 
for fair comparisons,
we conduct the evaluation on the divers motion synthesis from a \emph{single} example and disable the skeleton-aware motion patch extraction as described in Section~\ref{sec:patch_generation}.
%
We use three example sequences containing highly dynamic and agile movements for evaluation. The character consists of 65 joints, and each sequence has around 500 frames.
%
For each example sequence,
we use all methods to synthesize a novel sequence that doubles the length of the example.
%
% All experiments are conducted on a V100 GPU.


%

\paragraph{Qualitative Comparison}
\label{sec:comparisons}
%
%% we do not use the skeleton-aware component here for a fair comparison.
%% or, we should add a metric or user study to evaluate?
%
%% introduce comparison methods: MotionTexture, acRNN, GANimator
(i)
%% MotionTexture (only briefly)
% copy past from another paper is absolutely FORBIDDEN!!!!
To accomplish diverse motion synthesis, \emph{MotionTexture} organizes similar motion patches from training motions into linear dynamics models known as textons, and models the probability of transition between textons using a Markov Chain. 
%
However, it faces the challenge of balancing diversity and quality, particularly when there is only one example sequence due to the choice of linear dynamics model.
%
We follow the procedure as done in~\cite{ganimator} to apply MotinTexture to a single example.
%
As a result, MotionTexture produces unnatural transitions between textons.
(ii)
%
\emph{acRNN} uses an RNN-based network structure.
The lack of data leads to a model that is prone to overfitting and is not robust to perturbation or error accumulation.
Consequently, acRNN can only stably generate a limited number of frames.
(iii)
%% GANimator 
\emph{GANimator} utilizes a series of GANs to capture the distribution of motion patches at different scales, in order to progressively synthesize motions that closely resemble the input.
%
In our experiments with complex and large skeletons, as shown in \Cref{tab:differentskeletons}, GANimator struggles to produce high-quality results, often resulting in jittery or over-smoothed motions. Additionally, it requires a significant amount of training time, typically from several hours to a day.
%
%% All neural-based methods
%The neural-based methods need ad-hoc designs to extract features from motion data and can not handle complex skeletons due to \wy{gradient vanishing issue (I'm not sure)}, moreover, the smoothness of the neural network makes it difficult to synthesize motions with high-frequency details.
%
In contrast,
our method can adapt to these complex skeletal structures and various motion styles, and synthesize diverse and high-quality variations as shown ~\Cref{fig:comparisons}.
Notably, highly dynamic motions, in particular sharp and agile movements, are well preserved in our synthesized results. 
%\plc{I would be very careful about this. Because it somehow relates me to music guided dancing generation and those people are quite picky about rhythmic movements. I would rather say that we preserve the dynamics of the motion.}
For more qualitative results, please refer to the accompanying video.
%

%
% \todo{update with a comparison figure.}



%
%% only briefly introduce metrics for evaluation
\paragraph{Quantitative Comparison} Measuring the quality of generated results against a few examples is known to be difficult~\cite{ganimator}. 
%
As one of the pioneers, GANimator uses a combination of established metrics, namely coverage, diversity, and reconstruction loss, to rate the performance, since a single metric does not suffice the need of measuring the overall quality. 
%
However, the reconstruction loss is only suitable as a quality indicator for neural network-based methods. 
%
The diversity is measured with the average distance between generated motion patches and their nearest neighbor in the examples, and different motion patch size corresponds to local and global diversity. 
%
As a result, they tend to increase if the generated motion becomes unnatural, and favor results with minor perturbation or over-smoothed results generated by neural networks. 
%
We thus use neutral names for the diversity metrics, namely \emph{local patch distance} and \emph{global patch distance} in our experiments. 
%
We refer readers to \cite{ganimator} for more details about these metrics.
%
In addition, 
following the well-established metric in 2D image synthesis~\cite{singan}, %and 3D shape generation~\cite{achlioptas2018learning},
we also report the \emph{set diversity}, which measures the diversity among the generated results and is calculated as the averaged standard deviation of the rotation of each joint over 200 synthesized motions and normalized by the standard deviation of all joint rotations of the input example.
%
Note that, while this metric also has a preference for noisy output, we mainly rate the methods using the combination of the coverage and set diversity.


% \paragraph{Quantitative Comparison} Measuring the quality of the novel motion synthesis is known to be difficult when there is only one or a few examples~\cite{ganimator}. 
% %
% We adopt three metrics proposed by \citet{ganimator}, namely coverage, global diversity, and local diversity.
% %
% Nonetheless,
% it should be noticed that
% quantitatively evaluating the performance of a generative motion model is difficult.
% We are only able to rate methods using the \emph{combination} of these metrics,
% while none of these metrics alone suffices for the purpose.
% %
% In addition,
% the original local diversity in~\cite{ganimator},
% which actually measures the average distance between a local frame between its nearest neighbor frame in the example,
% can be interpreted as measuring either the local frame diversity or the opposite, local frame quality.
% %
% Thus, in this work, we use a neutral name for this metric \--- \emph{local distance}. 
% %
% %% diversity between samples
% Furthermore,
% as the global diversity in~\cite{ganimator} only measures the diversity inside a single generated motion,
% to evaluate the diversity of a set of generated motions, following~\cite{singan}, 
% we propose to measure the \emph{set diversity},
% which is calculated as the averaged standard deviation (std) of the rotation of each joint over 200 synthesized motions and normalized by the std of all rotations of the input example.

\input{table/single_motion_gen.tex}

%
The quantitative comparison results are shown in Table~\ref{tab:single_motion_gen}.
Notably,
our method produces a significantly high coverage score, while still exhibiting sufficiently diverse results (evidenced by a high set diversity score). For a more comprehensive comparison of the quality, we refer the readers to the accompanying video.
%
Note, we also report the computation time in \Cref{tab:single_motion_gen}, where we can see that our method is highly efficient, as it is both training-free and extremely fast during inference.
%




\if 0

%
%% single motion sequence: Gangnam-style, Ailing-dance, hip-hop-dance
\paragraph{Generation from A Single Exemplar}
% compare our methods in the default setting (with 65 joints) and 2 times length of the training frames
We use different types of motion for extensive evaluation, and collect 3 motion sequences which include fashion modern dance and hip-hop. 
The number of joints for the character is 65 and each sequence are around 500 frames at 30 fps.
For each sequence, we synthesize a novel sequence with 2 times the lengths of the input example.
%
%% MotionTexture
We manually pick a path to generate a novel motion for MotionTexture (as in GANimator), it produces unnatural transitions between textons due to the lack of sufficient data for statistical modeling.
%
%% MotionTexture(single) 
We also use the whole input as a single texton, which only synthesizes the same motion as in the exemplar due to the absence of global transition probability. \wy{Only local LDS. We can validate using the diversity over samples.}
%
%% acRNN
acRNN produces noisy motions in some data and others quickly converge to a static pose.
\wy{(acRNN using xyz position of each joint to represent motion and convert to rotation, the inverse IK is not stable and failed on many datasets)}
%
%% GANimator
The performance of GANimator~\cite{ganimator} drops sharply as the number of joints of the character increase.
GANimator produces over-smooth motions, especially in hip-hop data, and needs a long training time that increases linearly by the length of the input.
\fi

%
%% More Experiments
\subsection{More Evaluations}
\label{more_experiments}
%
In addition to the basic setting used above,
we further evaluate our method in the following aspects.

\paragraph{Skeleton-aware Motion Patches.}
%
In addition to the temporal axis, our method is also able to extract motion patches from examples along the skeletal axis, thus allowing obtaining diversity also on the spatial dimension as shown in \Cref{fig:skeleton_aware} and the accompanying video.
%
%
% Figure~\ref{fig:skeleton_aware} presents the results, where
% the skeleton is partitioned into overlapping skeletal parts manually by an artist,
% and the gain of enabling the skeleton-aware motion patch extraction is demonstrated.


\paragraph{Multiple Examples.}
%% WHY we do this exp.
Unlike existing methods, 
which struggle when presented with multiple example sequences due to the lack of explicit encouragement of completeness,
our method can handle multiple examples with the completeness control knob in Equation~\ref{eq:distance_metric}.
%% HOW to do this
We collect five dancing sequences ranging from 120-220 frames at 30 fps. It can be seen in \Cref{tab:multimotiongencoverage} that when more examples are given, existing methods generate results with lower coverage while our method remains a high coverage.
%
% We adapt each method to generate motions using 2 to 5 examples and report the coverage score averaged over multiple examples.
%
% Table~\ref{tab:multimotiongencoverage} presents the quantitative results.
%
%% Conclusions
MotionTexture produces unnatural transitions, similar to its results in the single-example setting.
%
acRNN fails on the task and produces noisy motions due to the diverse but scarce motion data.
%
GANimator requires a corresponding pre-defined latent variable for each sequence. However, the structure of the given sequences is not taken into consideration for defining these latent variables, hindering the network from generating various and complete samples.
%
In contrast,
our method 
%can use a small $\alpha$ to encourage the use of motion patches from all examples, eventually producing 
produces motions that cover a large portion of the examples with a properly set completeness control knob as shown in \Cref{fig:coverage} and the accompanying video.
% \xl{need a figure.}



\if 0
%% 
The skeleton-aware component gives us an opportunity to generate diverse motions not only on the temporal dimension but also on the spatial. 
%
%% HOW to do this
We can manually split the skeleton into different parts and synthesize the motion of each part individually.
Figure \todo{TBD} presents the results, the movements of the hands are synchronized in the input exemplar, while we can generate punch motion.
\fi



\if 0

%% multiple motion sequences: 
\paragraph{Generation from Multiple Exemplars}
% \xl{
% 1. to wy, write more details.
% 2. add a figure to show the coverage of multiple exemplars, possibly with a comparison.
% }
%
%% WHY we do this exp.
Previous methods have no mechanism to guarantee the even use of all input examples.
%
%% HOW to do this
To validate the explicit completeness knob, we collect five dancing sequences ranging from 120-220 frames of 30 fps.
Each method is trained individually using 2 to 5 exemplars and we report the average coverage score over examples.
%
%% Conclusions
MotionTexture also produces unnatural transitions as in single motion generation.
acRNN produces noisy motions due to the diverse \wy{compare to single setting} and insufficient motion data.
GANimator does not have any component to guarantee the coverage and performance drops sharply as the number of input samples increases.
Ours can manually control the opportunity of the use for each input example and enforce the completeness of the synthesized motions.
\fi


\paragraph{Complex Skeletons.}
% In addition to the 65-joint skeletons used in Section~\ref{sec:comparisons},
Our method can work with skeletons of high complexities (See Figure~\ref{fig:randomgenetaion}),
on which the GAN-base method GANimator fails to produce reasonable results as demonstrated in the accompanying video.
%
Specifically,
we experiment with skeletons consisting of 24, 65, and 433 joints.
%
It can be seen in \Cref{tab:differentskeletons} that GANimator performs normally on the 24-joint skeletons, while
its performance drops dramatically when presented with complex skeletons.
%
Whereas our method maintains a consistent performance for different skeletons,
evidenced by the fluttering effects of the skirt and dragon wings in the accompanying video.
%
% The quantitative results is reported in \Cref{tab:differentskeletons}.
%
\input{table/different_skeletons.tex}



\if 0


\paragraph{Contact Label.}
As aforementioned,
it is easy to incorporate contact labels and IK post-process into our framework, to further mitigate rare foot sliding artifacts, particularly in the synthesis with large root-motion examples.
%
The visual results are presented in ??.
\xl{to be finalized.}


\paragraph{The Complexity of Skeletons}

%
%% 
%
%% conclusion -> WHY? Maybe the gradient vanishing
\wy{I think we need to explain WHY the NN-based methods can not handle the complex skeletons. Peizhuo, do you have any idea?}
Neural-based methods struggle in handling complex skeletons and meet critical performance degradation issues as the number of joints increases as shown in Table~\ref{tab:differentskeletons}.
%
%% HOW to do.
%
%% For the same motion, using different complexity of skeletons.
For the synthesis using 24 and 65 joints, we use the sample motion sequence (Samba dance) as input 
and then manually remove some joints of the character to reduce the number of joints from 65 to 24.
%
%% Conclusion
The performance of GANimator drops sharply when the number of joints increases using the same movements, 
while ours have no sudden degradation.
%
%% For a more complex skeleton
We also collect a motion with a more complex skeleton (with 433 joints) from real production work.
\wy{can we address the real-world usage? To show that complex skeletons are used in real production commonly.}
GANimator almost fails to synthesize novel motions and produces drunk motions.
Ours can generate plausible results with highly motion details.
Table~\ref{tab:differentskeletons} shows the numerical results of the effect of the number of joints.
\fi

% %
% %% Maybe the hierarchical structure leads to sparse/small gradients of the leaf joints?
% \xl{
% 1. ours and ganimator on various skeletons: 24, 65, 433 joints.
% 2. no visual figure (for now)
% 3. only a table
% }


\if 0
\paragraph{Rotation Representation}
\label{rotationrepresentation}
% Our framework is robust to different rotation representations, 
% which plays an important role in neural-based methods.
\input{table/different_rotations.tex}
\fi

\if 0

\paragraph{Details Preservation}
\label{motiondetails}
A particular feature of our patch-based method is the preservation of details of examples.
Rhythmic motions like hip-hop and jumping can be obtained in the synthesized results.
%
%% Maybe we need to explain WHY the NN-based methods produce motions without details?
% Neural-based methods
As evidenced in Figure~\ref{fig:randomgenetaion}, our methods can preserve the high-frequency details in exemplars, 
such as the jittered wings of the dragon and the sense of the rhythm of dancing.
We refer readers to the accompanying video.
\fi

% \wy{I want to add a figure of the velocity of the end joint to show this point.}
% \xl{
% 1. on two example sequences (dragon and hip-hop dance)
% 2. say what is good with ours
% 3. refer to the supplementary video.
% 4. (optional) a curve figure.
% }



==> submission/5-applications.tex <==
\section{Applications}
%
%
%% =========================================================================
%% bullet points:
%%       1) skeleton-aware component =====> Reassembly / Motion Completion
%%       2) explicit editing         =====> Endless Looping / Motion Completion
%% =========================================================================

%
%% 
In this section, we demonstrate the versatility of our framework
by adapting it to various applications,
such as motion completion,
key frame-guided generation, infinite looping, and motion reassembly.
% More implementation details can be found in the supplementary.
% 
The results are presented in \Cref{fig:applications}. A more detailed demonstration is available in the accompanying video.



\paragraph{Motion Completion.}
Our framework, which utilizes skeleton-aware motion patch extraction, enables the completion of partial motions that contain only the movement of specific body parts.
%
For example,
when a lower-body motion sequence $\partialmotion^{\text{lower}}$ is provided,
the upper-body motion can be completed using the example motion.
%
%% HOW to do 
Specifically,
we build a pyramid for the partial-body motion 
$\{ \partialmotion^{\text{lower}}_1, ...,  \partialmotion^{\text{lower}}_\nbstage \}$,
and the corresponding partial motion in the output $\motionfeatout_s$ is fixed to $\partialmotion^{\text{lower}}_\idstage$ at each stage $\idstage$.
%
Our framework then automatically synthesizes the movements of the rest by parts, 
completing the partial constraints with a coherent and natural motion.
%(See Figure~\ref{}).
% the specific partial-body motion $\partialmotion^{lower}$ 
% This is realized by fixing the specific partial-body motion $\partialmotion^\nbpart$ 
% during multi-scale synthesis.


\paragraph{Key Frame-guided Generation.}
Our method also allows users to manually specify a sparse set of key frames to guide the content of the synthesized motion. Our method can then effectively handle these sparse pose constraints distributed throughout the sequence and generate smooth, highly-detailed motion.
% Users can manually specify a sparse set of key frames to guide the content of the synthesized motion,
% then our method can cope with these sparse poses distributed along the whole sequence
% and produce smooth, highly-details motion.
%\wy{It is complicated if we introduce more symbols, so I just clarify the main pipeline.}
%
%% HOW to do 
Given a set of key frames at the coarsest stage, 
we replace corresponding frames in $\motionfeatout_1$ with the specified frames,
and fix them through the whole generation process.


\paragraph{Infinite Looping.}
Our framework can easily synthesize endless looping motion by fixing the ending pose to be identical to the beginning pose at every stage in the synthesis. This allows for the seamless looping of the entire motion sequence. It can be useful in animation production, such as creating repetitive crowds like spectators cheering outside an arena.


% Our framework can synthesize endless looping motion with an easy twist.
% %which is non-trivial for RNN-based methods as they rely on the previous prediction, 
% %and for fully convolutional neural networks as they need ad-hoc designs, such as additional loss constrain, during training.
% We achieve this via simply fixing the ending pose to be identical with the beginning pose at every stage in the synthesis,
% and thus we can loop the whole motion sequence over and over.
% This can be useful in animation production, such as creating spectators cheering outside the arena.
%% HOW to do 
%We realized this by adding virtual patches 
%containing the beginning and the end of the motion frames 
%and then optimizing the virtual patches to be continuous at each stage. \wy{Or to say, match a coherent motion patch.} 

% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=\linewidth]{image/application_endless_looping.pdf}
%   \caption{Endless looping results. 
%   }
%   \label{fig:endlesslooping}
% \end{figure}

\paragraph{Motion Reassembly.}
%\wy{I am working on this, so this is a very coarse draft.}
%As it is mentioned in Section~\ref{sec:more_setting}, our framework explicitly involves the skeletal structure for patch extraction, the skeletons across different motions do not necessarily be the same.
As aforementioned in \Cref{sec:more_setting}, our method has the ability to synthesize a Frankenstein. 
We demonstrate an example that stitches the right arm of a monster to a zombie; See~\Cref{fig:applications} and the accompanying video. Note the example sequence of these two characters is different and the zombie does not have any movement in its partially missing right arm, yet our method is still able to successfully synthesize a natural and meaningful motion.

% When motions of multiple creatures with different skeletons are given,
% our framework can take partial-body motions from each example and harmonize them to create a dynamic novel creature. 
% To achieve this, the user can split the skeleton of each input with overlap and manually specify the skeletal parts of interest to be used in the generative motion matching and blending. The overlapping region plays a crucial role in bridging different skeletal parts during the generation process. Our method then can synthesize the novel motion for the new creature by combining the partial-body motions as discussed in Section~\ref{sec:patch_generation}.
% So we can take the partial-body motion from each example, and harmonize them to create a dynamic novel creature. 
%
% To this end, 
% Given two motion sequences of two different creatures,
% we simply allow the user to split the skeleton of each input creature, and manually specify skeletal parts of interest
% to be used in the generative motion matching and blending.
%
%% HOW to do 
%Given two motion sequences with different skeletons $A$ and $B$, 
%users manually select the partial-body motion $\partialmotion^{A}$ and the partial-body motion $\partialmotion^{B}$,
% We then synthesize the novel motion for each skeletal part individually using the proposed framework, 
% and then combine them to form the final motion of a new creature.
%
%Figure~\ref{} presents the results using different motions with heterogeneous skeletons.

\input{table/multi_motion_gen_coverage.tex}






==> submission/6-conclusion.tex <==
\section{Discussion and Conclusion}
We presented a generative framework for synthesizing diverse motion sequences from only a small set of examples. 
%
We achieve this via injecting generative capabilities into the industry state-of-the-art technique for character animation \--- motion matching.
%
As a result,
our framework inherits the training-free nature and superior quality, 
and is able to produce a high-quality sample within just a fraction of a second, even with highly complex and large skeletons.
%
We demonstrate the
utility of our framework on a variety of applications. 
%
Despite its advantages, our method in its current form has a few shortcomings:
%
It uses a discrete patch distribution, whereas GANimator~\cite{ganimator} learns a continuous distribution. 
%
Therefore,
GANimator can generate novel poses with high likelihood from the learned distribution.
%
Although the skeleton-aware component can be a remedy,
this capability is missing in our method. 
%
Nevertheless,
we argue that such generalization can be disadvantageous in motion synthesis, as sequences formed by novel poses often contain visual artifacts such as jittering and incoherence, which are highly noticeable to human eyes.
%
We prioritized the motion quality at the outset, which led us to  the motion matching approach.
%
%So the motion quality is given priority, and we try to mine
%
%And this priority on motion quality is what led us to motion matching at the outset.


Our method seeks to synthesize as many variants as can be mined from the examples,
rather than struggle to balance quality with novelty of motion.
%
As a consequence,
although diverse results of our method are shown,
the generative diversity of our method is lower than that of GANimator.
%
Hence,
a future work direction is to inject the high quality of motion matching into generative neural models, possibly with discrete neural representation learning techniques~\cite{van2017neural}, and thus obtain the best of both worlds. 
%
Last, 
our method cannot deal with overly long example sequences, as the normalized similarity matrices grow excessively large.
%
Adopting approximate nearest neighbors search, such as~\cite{patchmatch}, may help alleviate this issue.


\if 0
%%
\wy{

Strengths:
1:   very fast, and do not need training
2:   not data-driven, can learn from a single sequence
3:   do not need ad hoc designs
    3.1: robust to different rotation representation
    3.2: can handle complex skeletons (neural-based methods meet performance degradation issues when the skeleton are complex)
    3.3: previous works require desired and specific skeletal structure (not sure, mentioned in GANimator)
4:   completeness knob to enforce the use of all examples
5:   explicit editing

Weakness:
1:   hard to synthesize novel motion
2:   have to store motion patches, so can not handle a large number of motions
4:   similar to GANimator, the input exemplar must have multiple transition points
3:   can not continuously generation
5:   sometimes mode collapse

Limitations:
1:   our method struggles to synthesize natural motions when the contents of the input examples are largely different.

More bullet points:
1:   Do we really need more diversity in the single-motion generation? (Baoquan said that patch-based methods are conceptually more suitable for motion generation tasks at the last meeting.)
2.   Discuss like Drop-the-GAN
    2.1  the GAN-generated patch distribution behaves more like the reference distribution than the patch nearest neighbor-generated distribution, but with a loss of high-frequency details.
    
}

% \wy{Do we need to discuss the }
\xl{
1. we have less emphasis on generating absolutely novel poses.
but to mine as many diverse motions as possible from the exemplars.
this is different to ganimator.
}

\fi


==> submission/extra_figure_page.tex <==
\clearpage

%%%% visual comparison
\begin{figure*}[]
  \centering
  \includegraphics[width=\linewidth]{image/comparisons.pdf}
  \caption{
  Visual comparisons. 
  %We compare our method to classic and state-of-the-art deep learning techniques using a single sequence as input.
MotionTexture~\shortcite{motiontexture} generates motions with unnatural transitions. acRNN~\shortcite{acrnn} produces noisy motions or sometimes quickly converges to a static pose. GANimator~\shortcite{ganimator} struggles to handle complex skeletons, producing over-smoothing results. 
Our method outperforms these methods with diverse and high-quality results, where highly dynamic motions are well preserved. 
Please refer to the accompanying video for animation results.
  }
  \label{fig:comparisons}
\end{figure*}


%%%% skeleton-aware results
\begin{figure*}[]
  \centering
  \includegraphics[width=\linewidth]{image/skeleton_aware.pdf}
  \caption{The effectiveness of skeleton-aware motion patch extraction. 
  An artist manually divides the skeleton into three overlapping parts (top left).
  Given an example of a character waving two hands simultaneously, only a sequence with two waving hands can be synthesized without the skeleton-aware component. However, with the skeleton-aware motion patch extraction, a more diverse sequence, including waving with only one hand (in red boxes), can be generated.
  }
  \label{fig:skeleton_aware}
\end{figure*}



%%%% multiple examples
\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.95\linewidth]{image/coverage.pdf}
  \caption{
    Comparison under the multi-example setting.
    GANimator struggles to incorporate all examples, resulting in the loss of a significant portion of exemplar motion patches in the synthesis (marked in gray) and a low coverage score. In contrast, our method effectively covers all examples (marked as colorized), resulting in high coverage score. }
  \if 0
\wy{TBD}
  Coverage when using multiple examples. We visualize the \emph{Coverage} of each input example (labeled with highlight) for GANimator~\shortcite{ganimator} and our method. 
  GANimator ~\shortcite{ganimator} losses many contents if multiple examples as input,
  while ours can explicitly control the completeness of the synthesized motion.
\fi\label{fig:coverage}
\end{figure*}


\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.95\linewidth]{image/application_all.pdf}
  \caption{
  Applications.
  (1) Motion completion. Users can provide the lower-body motion (marked in yellow), and our method completes with diverse motions.
  (2) Key frame-guided generation. 
  Given a set of key frames (marked in red boxes), 
  we can generate diverse novel motion sequence that follow the key frame poses.
  (3) Infinite looping. 
  By simply specifying the starting and ending pose to be identical,
  our method can generate a infinitely looping animation, which can be useful in crowd simulation.
  (4) Motion reassembly. 
  Given two motion sequences with heterogeneous skeletons, our method can combine them to form a new creature with coherent and natural motion.
  }
  \label{fig:applications}
\end{figure*}

\clearpage

==> submission/math_utils.tex <==
% define all math-related symbols as global commands here

\newcommand{\nbframe}{ H }
\newcommand{\nbframein}{ T }
\newcommand{\nbframeout}{ F }
\newcommand{\nbjoint}{ J }
\newcommand{\rotdim}{ Q }
\newcommand{\realnum}{ \mathbb{R} }
\newcommand{\rootpos}{ \textbf{O} }
\newcommand{\rootdelta}{ \textbf{V} }
\newcommand{\jointrot}{ \textbf{R} }
\newcommand{\motionmetric}{ \mathcal{M} }
\newcommand{\motionfeatin}{ \textbf{T} }
\newcommand{\motionfeatout}{ \textbf{F} }


\newcommand{\nbstage}{ S }
\newcommand{\idstage}{ s }
\newcommand{\downsamplef}{ r }
\newcommand{\upsample}{ \uparrow^{ \downsamplef} }


\newcommand{ \patchsize }{ p }
\newcommand{\skeleton}{ \textbf{B} }
\newcommand{\skeletalpart}{ \bar{\skeleton} }
\newcommand{\nbpart}{B}
\newcommand{\idpart}{b}
\newcommand{\partialmotion}{ \bar{\motionfeatin} }

\newcommand{\qset}{ X }
\newcommand{\kset}{ Y }
\newcommand{\dist}{ D }
\newcommand{\simi}{ \hat{\dist} }

\newcommand{\nbiter}{ E }

\newcommand{\contactlabel}{ \textbf{L} }







\newcommand{\exemplar}{ E }
\newcommand{\synthesis}{ S }

\newcommand{\animatoin}{ A }
\newcommand{\partanimatoin}{ \overline{A} }
\newcommand{\bone}{ B }
\newcommand{\partbone}{ \overline{B} }
\newcommand{\foot}{ \mathcal{F} }
\newcommand{\motion}{ M }
\newcommand{\motionfeat}{ \mathcal{M} }
\newcommand{\partmotion}{ \overline{M} }
\newcommand{\partmotionfeat}{ \overline{\mathcal{M}} }
\newcommand{\nframe}{ T }
\newcommand{\nmotion}{ I }
\newcommand{\npart}{ N_b }
\newcommand{\nitr}{ N_{\text{step}} }
\newcommand{\ncontact}{ C }
\newcommand{\njoint}{ J }
\newcommand{\nrotfeat}{ K }
\newcommand{\rotation}{ \textbf{R} }
\newcommand{\translation}{ \textbf{O} }
\newcommand{\velocity}{ \textbf{V} }


\newcommand{\upsampleratio}{ r }

\newcommand{\stride}{ s }





==> table/different_rotations.tex <==
\begin{table}[b!]
\caption{
%% SambaDancing
Different rotation representations.
\wy{Deprecated}
% \wy{Finished. The coverage of ganimator using quaternion is kind of wired. I have checked the poor visual quality, we may mention readers to refer the video }
}
\footnotesize
\setlength{\tabcolsep}{1.5pt}
\centering

\begin{tabular}{llcc} 
\toprule
 &  & 6D Representation~\shortcite{zhou6d} & Quaternion \\ 
\midrule
\multirow{3}{*}{GANimator~\shortcite{ganimator}} & Coverage$\uparrow$  & 44.10 & 99.90 \\
 & Global Diversity & 2.02 & 1.10 \\
 & Local Diversity & 1.94 & 1.03 \\ 
\midrule
\multirow{3}{*}{Ours} & Coverage$\uparrow$ & 99.84 & 99.32  \\
 & Global Diversity & 0.15 & 0.08 \\
 & Local Diversity & 0.15 & 0.08 \\
\bottomrule
\end{tabular}

\label{tab:differentskeletons}
\end{table}%


==> table/different_skeletons.tex <==
\begin{table}[t!]
\caption{
%
%% SambaDancing, SambaDancing, VN_cha_WuDao_dy_qhc002_T005_cha_125_986
% \wy{TBD}
Coverage rate on skeletons with different complexity.
% Our method works well with highly complex skeletons, whereas the performance of GANimator drops dramatically.
% Coverage scores are reported in the table.
}
\footnotesize
\setlength{\tabcolsep}{8pt}
\centering

\begin{tabular}{lccc} 
\toprule
 & \multicolumn{3}{c}{Number of Joints} \\ 
\cline{2-4}
 &  24 & 65 & 433 \\ 
\midrule
GANimator~\shortcite{ganimator} & 92.10 & 44.10 & 2.38 \\
% \midrule
Ours & 97.82 & 99.84 & 86.90 \\
\bottomrule
\end{tabular}

\vspace{-8px}

\label{tab:differentskeletons}
\end{table}%


==> table/different_skeletons_bak.tex <==
\begin{table}[b!]
\caption{
%
%% SambaDancing, SambaDancing, VN_cha_WuDao_dy_qhc002_T005_cha_125_986
The effect of the number of joints of a skeleton.
% \wy{Finished. We may not report the diversity? Because the score dose not reflect the real quality.}
% \xl{remove diversity scores.}
}
\footnotesize
\setlength{\tabcolsep}{8pt}
\centering

\begin{tabular}{llccc} 
\toprule
 &  & \multicolumn{3}{c}{Number of Joints} \\ 
\cline{3-5}
 &  & 24 & 65 & 433 \\ 
\midrule
\multirow{3}{*}{GANimator~\shortcite{ganimator}} & Coverage$\uparrow$ & 92.10 & 44.10 & 2.38 \\
 & Global Diversity & 1.56 & 2.02 & 2.90 \\
 & Local Diversity & 1.48 & 1.94 & 2.81 \\ 
\midrule
\multirow{3}{*}{Ours} & Coverage$\uparrow$ & 97.82 & 99.84 & 86.90 \\
 & Global Diversity & 0.10 & 0.15 & 0.08 \\
 & Local Diversity & 0.10 & 0.15 & 0.09 \\ 
\bottomrule
\end{tabular}

\label{tab:differentskeletons}
\end{table}%


==> table/hyperparameters.tex <==
\begin{table}[t!]
\caption{
The different settings of hyperparameters.
}
\footnotesize
\setlength{\tabcolsep}{1.5pt}
\centering

\begin{tabular}{lccccc} 
\toprule
 & Coverage & Set Diversity & Global Patch Dist. & Local Patch Dist. \\ 
\midrule
Ours (not use $\alpha$) & 87.45 & 0.27 & 0.18 & 0.17 \\
Ours ($\alpha = 5$) & 87.89 & 0.27 & 0.18 & 0.17 \\
Ours ($\alpha = 0.5$) & 88.47 & 0.27 & 0.18 & 0.17 \\
Ours ($\alpha = 0.05$) & 93.80 & 0.27 & 0.18 & 0.17 \\
Ours ($\alpha = 0.005$) & 99.96 & 0.27 & 0.30 & 0.23 \\ 
Ours ($\alpha = 0.0$) & 36.78 & 0.25 & 2.17 & 1.60 \\ 
\midrule
Ours ($K = 20$) & 87.74 & 0.25 & 1.03 & 0.71 \\
Ours ($K = 15$) & 92.04 & 0.26 & 0.73 & 0.54 \\
Ours ($K = 10$) & 96.07 & 0.27 & 0.42 & 0.36 \\
\midrule
Ours ($\patchsize = 23$) & 99.85 & 0.26 & 0.27 & 0.24 \\
Ours ($\patchsize = 17$) & 99.88 & 0.26 & 0.23 & 0.21 \\
Ours ($\patchsize = 5$) & 99.66 & 0.27 & 0.41 & 0.32 \\
\midrule
Ours ($\downsamplef = 2$) & 99.61 & 0.27 & 0.22 & 0.20 \\
Ours ($\downsamplef = 4$) & 99.16 & 0.27 & 0.34 & 0.28 \\
Ours ($\downsamplef = 8$) & 97.97 & 0.26 & 0.57 & 0.42 \\ 
\bottomrule
\end{tabular}

\label{tab:hyperparameters}
\end{table}%


==> table/multi_motion_gen_coverage.tex <==
\begin{table}[t!]

\caption{
% Quantitative comparison on multiple example-based generation.
Coverage rates of different numbers of example sequences.
%\wy{We may need to mention 'the average Coverage over all exemplars' here.}
%Average \emph{Coverage} of generation from multiple exemplars.
}
\footnotesize
\setlength{\tabcolsep}{3pt}
\centering

\begin{tabular}{lcccc} 
\toprule
 & \multicolumn{4}{c}{Number of Example Sequences} \\ 
\cline{2-5}
 & 2 & 3 & 4 & 5 \\ 
\midrule
MotionTexture~\shortcite{motiontexture} & 100 & 29.19 & 10.03 & 27.69 \\
acRNN~\shortcite{acrnn} & 7.34 & 4.02 & 1.38 & 0.41 \\
GANimator~\shortcite{ganimator} & 63.55 & 23.90 & 17.30 & 16.22 \\
Ours & 99.71 & 99.95 & 99.91 & 99.64 \\
\bottomrule
\end{tabular}

% \vspace{-20px}
\label{tab:multimotiongencoverage}
\end{table}%


==> table/single_motion_gen.tex <==
\begin{table}[t!]
\caption{
Quantitative comparisons on single example-based generation.
% \xl{name and order: Set diversity, Coverage, Global diversity, Local distance}
%\plc{It's too crowded. If we have time (and space), split the running time into another table.}
% \xl{to pl, check the time for motiontexture.}
}
\footnotesize
\setlength{\tabcolsep}{1.6pt}
\centering

\begin{tabular}{lcccccc} 
\toprule
  & Coverage & \begin{tabular}[c]{@{}c@{}}Set \\Div.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Global \\Patch Dist.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Local \\Patch Dist.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Training\\Time \end{tabular} & \begin{tabular}[c]{@{}c@{}}Inference\\Time \end{tabular} \\ 
\midrule
MotionTexture~\shortcite{motiontexture} & 84.12 & 0.05 & 1.12 & 1.13 & 32.3s & 0.03s \\
MotionTexture (Single) & 100.00 & 0.01 & 0.45 & 0.44 & 0.08s & 0.07s \\
acRNN~\shortcite{acrnn} & 5.13 & 0.75 & 13.62 & 13.55 & 25 hrs & 0.21s\\
GANimator & 49.07 & 0.24 & 2.18 & 2.08 & 6 hrs & 0.12s\\
Ours & 99.89 & 0.28 & 0.22 & 0.18 & N/A & 0.08s\\ 
\bottomrule
\end{tabular}

\label{tab:single_motion_gen}
\end{table}%

